Text Classification via Large Language Models

Despite the remarkable success of large-scale Language Models (LLMs) such as GPT-3, their performances still significantly underperform fine-tuned models in the task of text classification. This is due to (1) the lack of reasoning ability in addressing complex linguistic phenomena (e.g., intensification, contrast, irony etc); (2) limited number of tokens allowed in in-context learning. In this paper, we introduce Clue And Reasoning Prompting (CARP). CARP adopts a progressive reasoning strategy tailored to addressing the complex linguistic phenomena involved in text classification: CARP first prompts LLMs to find superficial clues (e.g., keywords, tones, semantic relations, references, etc), based on which a diagnostic reasoning process is induced for final decisions. To further address the limited-token issue, CARP uses a fine-tuned model on the supervised dataset for $k$NN demonstration search in the in-context learning, allowing the model to take the advantage of both LLM's generalization ability and the task-specific evidence provided by the full labeled dataset. Remarkably, CARP yields new SOTA performances on 4 out of 5 widely-used text-classification benchmarks, 97.39 (+1.24) on SST-2, 96.40 (+0.72) on AGNews, 98.78 (+0.25) on R8 and 96.95 (+0.6) on R52, and a performance comparable to SOTA on MR (92.39 v.s. 93.3). More importantly, we find that CARP delivers impressive abilities on low-resource and domain-adaptation setups. Specifically, using 16 examples per class, CARP achieves comparable performances to supervised models with 1,024 examples per class.

==> ablation_freq_avg.tex <==
\begin{table}[t]
    \centering
    \small
    \scalebox{0.8}{
    \begin{tabular}{l|ccc|c|ccc}\toprule
    & \multicolumn{2}{c}{\textbf{\it SST-2}} & & \multicolumn{3}{c}{\textbf{\it R8}}\\\midrule
    {\bf $k$-shot} & {\bf FT freq} & {\bf FT freq} & {\bf overlap avg} & & {\bf FT freq} & {\bf overlap avg} \\\midrule
    24 & 5516  &  2.38 & & 4242   & 5.16\\
20 & 5243  &  1.88& & 4073  &  4.11\\
16 & 4831  &  1.40& & 3860  &  3.08\\
12 & 4268  &  0.96& & 3536  &  2.16\\
8  & 3392  &  0.56& & 2985  &  1.29\\
4  & 1948  &  0.22& & 1968  &  0.55\\
2  & 940& 0.10& &1139  &  0.24\\
\bottomrule
    \end{tabular} 
    }
    \caption{The effect of Look-Around on other NAT models.}
\label{table:freq_demo_set}
\end{table}

==> ablation_freq_demo_details.tex <==
\begin{table*}[t]
    \centering
    \small
    \scalebox{0.9}{
    \begin{tabular}{lccccccccccccc}\toprule
    & \multicolumn{7}{c}{\textbf{\it SST-2}} & \multicolumn{6}{c}{\textbf{\it R8}}\\\midrule
    {\bf $k$-shot} & {\bf Mean} & {\bf 1}  & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} & & {\bf Mean} & {\bf 1}  & {\bf 5} & {\bf 10} & {\bf 15} & {\bf 20} \\\midrule
   & \multicolumn{7}{c}{{\bf FT $k$NN-Sampler}} &  \multicolumn{6}{c}{{\bf FT $k$NN-Sampler}}\\\midrule
24 & 7.19&	6081	&3209	&1505	&748	&397&&11.63	&4516	&3094	&1931	&1259	&828\\
20&	6.17&	5904	&2772	&1134	&521 	&282&&9.89&	4426	&2805&	1624	&989	&593\\
16&	5.16	&5644&	2278&	784&	335	&139&&8.17	&4287	&2420	&1252	&696	&386\\
12&	4.14	&5276&	1649&	477	&166&	47&&6.41	&4101	&1930	&876	&412&	195\\
8&	3.16&	4615	&950	&201	&46	&16&&4.69	&3730	&1286	&465	&180&	73\\
4&	2.12	&3434&	293	&29	&5&	1&&2.99	&2928&	546	&117	&32	&11\\
2&	1.61&	2260&	61&	1	&1&	0&&2.10	&2086	&171&	22	&7	&3\\\bottomrule
& \multicolumn{7}{c}{{\bf SimCSE $k$NN-Sampler}} & \multicolumn{6}{c}{{\bf SimCSE $k$NN-Sampler}}\\\midrule
24	&7.06	&6193	&3052	&1411	&736	&426&&11.61	&4525	&2949&	1701&	1065	&705\\
20	&6.03	&6036	&2604	&1092	&542	&283&&9.92	&4414&	2631	&1422	&838	&539\\
16	&5.03	&5789	&2111	&798	&349	&156&&8.20	&4271	&2244&	1102	&610	&383\\
12	&4.05	&5393	&1554	&483	&175	&66&&6.51	&4034&	1773	&758&	393	&236\\
8	&3.04	&4789	&905	&210	&49	&17&&4.82	&3636&	1180	&433&	202	&112\\
4	&2.06	&3534	&277	&31	&4	&0&&3.11&	2816	&536	&130	&54	&27\\
2	&1.55	&2355	&52	&0	&0	&0&&2.20	&1987&	178	&35	&11	&3\\
\bottomrule
    \end{tabular} 
    }
    \caption{The effect of Look-Around on other NAT models.}
\label{table:freq_demo}
\end{table*}

==> algorithm.tex <==
\algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
\algrenewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\To}{{\bf to }}
\newcommand{\IF}{{\bf if }}
\newcommand{\DO}{{\bf do }}
\newcommand{\ENDIF}{{\bf endif}}
\begin{algorithm}[t]
\small
\begin{algorithmic}
\Require sentence $s$, 
 EntityQuesTemplates, RelQuesTemplates
\Ensure a list of triples M = [rel$(e_1, e_2)]$
\State
\State $M \gets \emptyset$
\State  HeadEntList$\gets \emptyset$
\For {entity\_question in EntityQuesTemplates}
  \State $e_1$ = Extract\_Answer(entity\_question, s)
  \State \IF $e_1\neq \textsc{None}$  \DO \\ 
  %\hspace{0.7cm}  HeadEntList = HeadEntList +  $\{e_1\}$\\
   \hspace{0.7cm}  HeadEntList = HeadEntList +  $\{e_1\}$
   \State \ENDIF
 \EndFor
 \State
 \For {head\_entity in HeadEntList}
 \For {(rel, rel\_template) in RelQuesTemplates}
\State rel\_question = f (head\_entity, rel\_template)
  \State $e_2$ = Extract\_Answer(rel\_question, s)
  \State \IF $e_2\neq \textsc{None}$  \DO \\ 
  \hspace{1.2cm}  M = M +  [rel$(e_1, e_2)$] 
     \State \ENDIF
 \EndFor
 \EndFor
 \State
\State \Return $M$
\end{algorithmic}
\caption{Transforming the entity-relation extraction task to a multi-turn QA task.}
\label{alg}
\end{algorithm}

==> prompt_example.tex <==
\begin{table*}
\label{tab:methods}
\centering
\small
\vskip 0.1in
\scalebox{0.95}{
\begin{tabular}{ll}
    \toprule
    {\bf \textit{Data}} & \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Test: & <{\bf text:} "I like cats.", {\bf annotated sentimental polarity:} positive>  \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Demonstration: & <{\bf text:} "Dogs are cute.",  {\bf annotated sentimental polarity:} positive> \\\midrule
    {\bf \textit{Task Description}} & \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Classify: & Classify the sentiment of the input sentence as positive or negative. \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Explain-Classify: & First, list clues and explain the reasoning process for determination. \\
    & Next, based on the explanation, classify the sentiment as positive or negative. \\
    %&  classify the sentiment as positive or negative.\\ 
    \midrule
    {\bf \textit{Classify Prompts}} & \\ 
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Zero-shot Prompt: & Classify the sentiment of the input sentence as positive or negative. \\
    & {\bf INPUT}: I like cats. \\ 
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    One-shot Prompt: & Classify the sentiment of the input sentence as positive or negative. \\
    &  \\
    & {\bf INPUT}: Dogs are cute. \\ 
    & {\bf SENTIMENT}: positive \\
    &  \\
    & {\bf INPUT}: I like cats. \\ 
    \midrule
    {\bf \textit{Explain-Classify Prompts}} & \\ 
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Zero-shot Prompt: & First, list clues and explain the reasoning process for determination. \\
    & Next, based on the explanation, classify the sentiment as positive or negative.\\ 
    & {\bf INPUT}: I like cats. \\ 
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    One-shot Prompt: &  First, list clues and explain the reasoning process for determination. \\
    & Next, based on the explanation, classify the sentiment as positive or negative.\\ 
    &  \\
    & {\bf INPUT}: . \\ 
    & {\bf CLUES}: 1. The phrase "Dogs are cute" implies a favorable opinion about dogs. \\
    & 2. The adjectives used to describe the subject (dogs) are generally associated with positive sentiment. \\
    & 3. The sentence does not contain any negative words or phrases that would suggest a negative sentiment. \\
    & Reasoning Process: Based on the clues and the lack of negative words or phrases, it is reasonable \\
    & to conclude that the sentiment of the sentence is positive. \\
    & {\bf Sentiment}: positive \\
    &  \\
    & {\bf INPUT}: I like cats. \\ 
    %\midrule
    \bottomrule
\end{tabular}
}
\caption{Examples of prompts for setups in Section~\ref{sec:methods}.}
\label{example:prompt}
\end{table*}


==> prompts_agnews.tex <==
\begin{table*}
\label{tab:methods}
\centering
\small
\vskip 0.1in
\scalebox{0.95}{
\begin{tabular}{ll}
    \toprule
    \multicolumn{2}{c}{\bf AGNews : topic classification} \\
    \toprule
    {\bf \textit{Label Word Map}} & \{1: World,
      2: Sports,
      3: Business,
      4: Sci/Tech\} \\\midrule
    {\bf \textit{Zero-Shot}} & \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Classify Prompt: & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\ 
    & INPUT: <sent> \\
    & SENTIMENT:  \\
    %& \text{} \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Reason-Classify Prompts: & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\
    & INPUT: <sent> \\
    & \text{} \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Findclue-Reason-Classify & {\bf Step 1:} \\
    & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative.\\ 
    & INPUT: <sent> \\
    & \text{} \\
    & {\bf Step 2:}\\ 
    & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\ 
    & INPUT: <sent> \\
    & CLUES: <step-1-response>\\
    & \text{} \\
    \midrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % few-shot 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    {\bf \textit{Few-Shot}} & \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Classify Prompt: & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\ 
    & INPUT: <demo-sent> \\
    & SENTIMENT: <demo-label-word> \\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & SENTIMENT: <demo-label-word> \\
    & \text{} \\
    & INPUT: <sent> \\
    & SENTIMENT:  \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Reason-Classify Prompts: &  {\bf Step 1:}\\
    & Classify the sentiment of the input sentence as positive or negative. \\
    & INPUT: <demo-sent> \\
    & \text{} \\
    & {\bf Step 2:} \\ 
    & Classify the sentiment of the input sentence as positive or negative.  \\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <test-sent> \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Findclue-Reason-Classify Prompts: &  {\bf Step 1:}\\
    & Classify the sentiment of the input sentence as positive or negative. \\
    & INPUT: <demo-sent> \\
    & \text{} \\
    & {\bf Step 2:} \\ 
    & Classify the sentiment of the input sentence as positive or negative.  \\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <test-sent> \\
    %%%%%%%%%%%%%%%%%%%%%
    %\midrule
    \bottomrule
\end{tabular}
}
\caption{Examples of prompts for setups in Section~\ref{sec:methods}.}
\label{example:prompt_agnews}
\end{table*}


==> prompts_r52.tex <==
\begin{table*}
\label{tab:methods}
\centering
\small
\vskip 0.1in
\scalebox{0.95}{
\begin{tabular}{ll}
    \toprule
    \multicolumn{2}{c}{\bf R52 : topic classification} \\
    \toprule
    {\bf \textit{Label Word Map}} & \{0: Unemployment,
      1: Interest Rates,
      2: Vegetable Oil,
      3: Capacity Utilisation,\\
    &  4: Balance of Payments, 
     5: Rubber,
      6: Leading Economic Indicators,
      7: Crude Oil,\\
    & 8: Strategic Metals, 
      9: Tin,
      10: Copper,
      11: Fuel Oil, 
      12: Meal Feed,\\
      & 13: Money Supply,
      14: Iron Steel, 
    15: Carcass,\\
   & 16: Instalment Debt/Consumer Credit,
      17: Lumber,
      18: Platinum, \\
    &  19: Natural Gas,
      20: Gross National/Domestic Product,
      21: Potato,
      22: Zinc, \\
    & 23: Tea,
      24: Retail Sales,
      25: Heating Oil/Gas Oil,
      26: Coffee, \\
    & 27: Grain, 
      28: Gasoline, 
      29: Orange,
      30: Sugar, \\
    &  31: Petro-Chemicals,
      32: Lead,
      33: Cotton, 
   34: Shipping,\\
   &  35: Nickel,
      36: Alum,
      37: Money/Foreign Exchange,
     38: Trade, \\
   & 39: Cocoa,
     40: Industrial Production Index,
     41: Wholesale Price Index,\\
   & 42: Reserves,
    43: Earnings and Earnings Forecasts,
    44: Acquisitions,\\
    & 45: Housing Starts, 
     46: Livestock,
     47: Consumer Price Index, \\
      & 48: U.S. Dollar,
      49: Gold, 
      50: Personal Income,
      51: Jet and Kerosene\} \\\midrule
    {\bf \textit{Zero-Shot}} & \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Classify Prompt: & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\ 
    & INPUT: <sent> \\
    & SENTIMENT:  \\
    %& \text{} \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Reason-Classify Prompts: & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\
    & INPUT: <sent> \\
    & \text{} \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Findclue-Reason-Classify & {\bf Step 1:} \\
    & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative.\\ 
    & INPUT: <sent> \\
    & \text{} \\
    & {\bf Step 2:}\\ 
    & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\ 
    & INPUT: <sent> \\
    & CLUES: <step-1-response>\\
    & \text{} \\
    \midrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % few-shot 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    {\bf \textit{Few-Shot}} & \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Classify Prompt: & Please classify the overall SENTIMENT polarity of the INPUT sentence as Positive or Negative. \\ 
    & INPUT: <demo-sent> \\
    & SENTIMENT: <demo-label-word> \\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & SENTIMENT: <demo-label-word> \\
    & \text{} \\
    & INPUT: <sent> \\
    & SENTIMENT:  \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Reason-Classify Prompts: &  {\bf Step 1:}\\
    & Classify the sentiment of the input sentence as positive or negative. \\
    & INPUT: <demo-sent> \\
    & \text{} \\
    & {\bf Step 2:} \\ 
    & Classify the sentiment of the input sentence as positive or negative.  \\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <test-sent> \\
    \specialrule{0em}{1pt}{1pt}
    \cdashline{1-2}
    \specialrule{0em}{1pt}{1pt}
    Findclue-Reason-Classify Prompts: &  {\bf Step 1:}\\
    & Classify the sentiment of the input sentence as positive or negative. \\
    & INPUT: <demo-sent> \\
    & \text{} \\
    & {\bf Step 2:} \\ 
    & Classify the sentiment of the input sentence as positive or negative.  \\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <demo-sent> \\
    & REASONING: <step-1-generated>\\ 
    & SENTIMENT: <demo-label-word>\\
    & \text{} \\
    & INPUT: <test-sent> \\
    %%%%%%%%%%%%%%%%%%%%%
    %\midrule
    \bottomrule
\end{tabular}
}
\caption{Examples of prompts for setups in Section~\ref{sec:methods}.}
\label{example:prompt_r52}
\end{table*}

